An Adaptive View of Adversarial Robustness from Test-time Smoothing Defense

The safety and robustness of learning-based decision-making systems are under threats from adversarial examples, as imperceptible perturbations can mislead neural networks to completely different outputs. In this paper, we present an adaptive view of the issue via evaluating various test-time smoothing defense against white-box untargeted adversarial examples. Through controlled experiments with pretrained ResNet-152 on ImageNet, we first illustrate the non-monotonic relation between adversarial attacks and smoothing defenses. Then at the dataset level, we observe large variance among samples and show that it is easy to inflate accuracy (even to 100%) or build large-scale (i.e., with size ~10^4) subsets on which a designated method outperforms others by a large margin. Finally at the sample level, as different adversarial examples require different degrees of defense, the potential advantages of iterative methods are also discussed. We hope this paper reveal useful behaviors of test-time defenses, which could help improve the evaluation process for adversarial robustness in the future.

==> sections/backup.tex <==
\subsubsection{Accuracy on adversarial examples and confidences on clean images}
We first focus on the relation between categorical accuracy on  adversarial examples ($h(g(x))$) and categorical confidences on clean images ($x$). 
One plausible assumption is that categories with higher confidences on clean images might be a bit harder for adversarial attacks. Hence, those categories may have higher accuracy after defense.
To validate this assumption, we take adversarial examples from two PGD attacks and perform anisotropic diffusion, bilateral filter, and mean filter as respective defense.
Contrary to the assumption, as categorical accuracy on adversarial examples increases (1st column in Figure \ref{fig:variance-among-categories}), there is no obvious trend in corresponding confidences on clean images (2nd column in Figure \ref{fig:variance-among-categories}). 
\begin{figure}
\centering  
\subfigure[Accuracy PGD ($\epsilon=0.01$) \label{subfig:categorical-accuracy_pgd-0.01}]{
\includegraphics[width=0.3\textwidth, trim={0 0 0 1.2cm}, clip]{figures/4.3/acc_001-0002.png}}
\subfigure[Confidence PGD ($\epsilon=0.01$)]{
\includegraphics[width=0.3\textwidth, trim={0 0 0 1.2cm}, clip]{figures/4.3/ad-confidence_001-0002.png}}
\subfigure[Ground-truth prob PGD ($\epsilon=0.01$)]{
\includegraphics[width=0.3\textwidth, trim={0 0 0 1.2cm}, clip]{figures/4.3/ad_pgd-001-0002_ground_truth_categorical_prob.png}}
\\
\subfigure[Accuracy PGD ($\epsilon=0.05$)]{
\includegraphics[width=0.3\textwidth, trim={0 0 0 1.2cm}, clip]{figures/4.3/acc_005-001.png}}
\subfigure[Confidence PGD ($\epsilon=0.05$)]{
\includegraphics[width=0.3\textwidth, trim={0 0 0 1.2cm}, clip]{figures/4.3/ad-confidence_005-001.png}}
\subfigure[Ground-truth prob PGD ($\epsilon=0.05$)]{
\includegraphics[width=0.3\textwidth, trim={0 0 0 1.2cm}, clip]{figures/4.3/ad_pgd-005-001_ground_truth_categorical_prob.png}}
\caption{\label{fig:variance-among-categories} Distribution of categorical accuracy on adversarial examples in increasing order (1st column), categorical confidence on clean samples (2nd column), and categorical probability at the ground-truth class (3rd column). (a)-(c): Results on adversarial examples that are generated from PGD ($\epsilon=0.01$), with anisotropic diffusion as defense. (d)-(f): same as (a)-(c) but the adversarial examples are generated from PGD ($\epsilon=0.05$). In each row, the order of categories (horizontal axis in all plots) are synchronized.} 
\end{figure}
\subsubsection{Accuracy on adversarial examples and probability assigned to ground-truth category}
Another assumption was made on the relation between accuracy and the initial probability assigned to the ground-truth category. Intuitively, it might be easier to defend an adversarial example with relatively higher probability assigned to the ground-truth category. 
However, such an intuition is disproved by the 3rd column in Figure \ref{fig:variance-among-categories}. 
% As two intuitive assumptions have failed to explain the large variance of categorical accuracy after defense, 
